Learning to Minimize the Remainder in Supervised Learning

The learning process of deep learning methods usually updates the model's parameters in multiple iterations. Each iteration can be viewed as the first-order approximation of Taylor's series expansion. The remainder, which consists of higher-order terms, is usually ignored in the learning process for simplicity. This learning scheme empowers various multimedia based applications, such as image retrieval, recommendation system, and video search. Generally, multimedia data (e.g., images) are semantics-rich and high-dimensional, hence the remainders of approximations are possibly non-zero. In this work, we consider the remainder to be informative and study how it affects the learning process. To this end, we propose a new learning approach, namely gradient adjustment learning (GAL), to leverage the knowledge learned from the past training iterations to adjust vanilla gradients, such that the remainders are minimized and the approximations are improved. The proposed GAL is model- and optimizer-agnostic, and is easy to adapt to the standard learning framework. It is evaluated on three tasks, i.e., image classification, object detection, and regression, with state-of-the-art models and optimizers. The experiments show that the proposed GAL consistently enhances the evaluated models, whereas the ablation studies validate various aspects of the proposed GAL. The code is available at \url{https://github.com/luoyan407/gradient_adjustment.git}.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> sec/sec_broader_impact.tex <==


\section*{Broader Impact}

This research studies a new learning paradigm that leverages information in the training steps to improve the descent. 
Being model agnostic and general, the method will advance and enrich the fundamental research in machine learning. The more efficient and effective search of local minimum that facilitates the learning process will also bring significant impacts in developing automatic systems in a wide range of domains including education, healthcare, e-commerce, and many more. As other machine learning methods, systems derived with the method may fall short in performance or interpretability. While the proposed method shows improved performance, depending on specific domains or applications with varied requirements, precautions may need to be taken accordingly before using the automatic systems. This work, targeting an generic learning framework rather than a specific task or application, does not foresee particular ethical concerns in any specific areas or societal consequences. For a broader impact, we release the software of our research to the public. The source code is %attached in the Supplementary Materials. It is also 
available at \url{https://rb.gy/qx1kuu}.


%This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. 
%This work is generic and its ultimate motivation is to benefit a broad variety of areas, \eg healthcare, education, economy, and etc, for human's material well-being.
%On the other hand, as the proposed method facilitates the learning process for applications, rather than implementing specific applications, 
%we believe that even the proposed work is modified for malevolent purposes, the resulting method would not harm humans and other morally relevant beings. 
%Because the proposed method is an essential tool for applications and is neutral to applications, and any modified version of this work cannot determine or re-shape the downstream applications. 
% In summary, this work has no direct link to malevolent applications.
%Therefore, this work does not present any foreseeable societal consequence.

% reference: The Ethics of Artificial Intelligence (published paper) and my imagination

%---------------previous version starts from here------------------
% This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. Our primary motivation is to provide a new perspective on the gradient descent that looks for a new direction to descend. The proposed method is generic and can apply to train models for other problems. As a result, the boosted model could used for both malicious and benevolent purposes. Nevertheless, the algorithmic impact of the proposed method has no direct link to malevolent applications and does not break the code of ethics.

% reference: https://hub.packtpub.com/machine-learning-ethics-what-you-need-to-know-and-what-you-can-do/

%---------------requirement starts from here------------------
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}
